Image-Based Dietary Assessment: A Healthy Eating Plate Estimation System

The nutritional quality of diets has significantly deteriorated over the past two to three decades, a decline often underestimated by the people. This deterioration, coupled with a hectic lifestyle, has contributed to escalating health concerns. Recognizing this issue, researchers at Harvard have advocated for a balanced nutritional plate model to promote health. Inspired by this research, our paper introduces an innovative Image-Based Dietary Assessment system aimed at evaluating the healthiness of meals through image analysis. Our system employs advanced image segmentation and classification techniques to analyze food items on a plate, assess their proportions, and calculate meal adherence to Harvard's healthy eating recommendations. This approach leverages machine learning and nutritional science to empower individuals with actionable insights for healthier eating choices. Our four-step framework involves segmenting the image, classifying the items, conducting a nutritional assessment based on the Harvard Healthy Eating Plate research, and offering tailored recommendations. The prototype system has shown promising results in promoting healthier eating habits by providing an accessible, evidence-based tool for dietary assessment.

==> name.tex <==
ADD
\textcolor{BrickRed}{} 

CORRECT
\colorbox{Dandelion}{orange background}

IDEA
\colorbox{Lavender}{IDEa is great}

{\color{RubineRed} hello

\rule{\linewidth}{0.5mm}}

https://www.sciencedirect.com/science/article/pii/S2161831323000935
https://www.cambridge.org/core/journals/proceedings-of-the-nutrition-society/article/new-mobile-methods-for-dietary-assessment-review-of-imageassisted-and-imagebased-dietary-assessment-methods/33E6AE4398065ACEBACE8E9E3AD170C9

